Computational discovery of bifunctional organic semiconductors for energy and biosensing

The discovery of synthetically accessible organic semiconductors with exceptional performance remains a critical bottleneck in materials science. While these materials offer compelling advantages - structural modularity, mechanical flexibility, and cost-effective solution processing - for applications in photovoltaics and biosensors, identifying candidates that balance high efficiency with practical synthesis presents significant challenges. To address this challenge, we developed a high-throughput screening approach using 17 458 molecules from the PubChemQC B3LYP/6-31G*//PM6 dataset. Our strategy employs a composite metric, PCESAScore = PCE - SAScore, which systematically balances power conversion efficiency (PCE) predictions from the Scharber model against synthetic accessibility scores. This approach successfully identified seven multi-functional candidates that demonstrate both exceptional photovoltaic performance (PCE up to 36.1 %) and strong protein-binding affinity for biosensing applications. Notably, molecule 4550 emerged as the optimal candidate, exhibiting a ligand efficiency of 0.340 kcal/mol/heavy atom with 100 % target promiscuity. Our computational framework integrates machine learning, density functional theory, and molecular docking to bridge the gap between theoretical performance and experimental feasibility. These findings establish a systematic pathway for discovering synthetically compatible organic semiconductors that can simultaneously address energy conversion and molecular recognition challenges.

==> Tables/table_correlations.tex <==
% AUTO-GENERATED: Correlations table (n=13) - 2026-01-29
% CRITICAL: Original correlation (r=-0.981, p=0.019) was SPURIOUS due to small sample (n=6)
% Expanded analysis (n=13) shows NO significant correlation
\begin{table}[h]
\centering
\caption{Pearson correlation coefficients for structure-property relationships in expanded dataset (n=13). The previously reported strong correlation between N in LUMO and $\lambda_{\text{hole}}$ (r=-0.981, p=0.019, n=6) was not robust to sample expansion, highlighting the importance of adequate statistical power.}
\label{tab:correlations}
\begin{tabular}{lcc}
\hline
Property Pair & Pearson $r$ & $p$-value \\
\hline
N in LUMO vs $\lambda_\text{hole}$ & -0.033 & 0.915 \\
N in HOMO vs $\lambda_\text{hole}$ & -0.089 & 0.773 \\
N in HOMO vs N in LUMO & 0.673 & 0.012* \\
\hline
\multicolumn{3}{l}{*Significant at $p < 0.05$ level} \\
\multicolumn{3}{l}{\textit{Note: Reorganization energy is governed by complex factors beyond N content.}} \\
\hline
\end{tabular}
\end{table}


==> Tables/table_correlations_old_n6.tex <==
\begin{table}[h]
\centering
\caption{Significant property correlations (p < 0.05). Pearson correlation coefficients between molecular properties.}
\label{tab:correlations}
\begin{tabular}{llccc}
\hline
Property 1 & Property 2 & n & Pearson r & p-value \\
\hline
N in HOMO (\%) & N in LUMO (\%) & 4 & 0.984 & 0.016 \\
N in LUMO (\%) & $\lambda_\text{hole}$ (eV) & 4 & -0.981 & 0.019 \\
\hline
\end{tabular}
\end{table}


==> Tables/table_functional_sensitivity.tex <==
\begin{table}[h]
\centering
\caption{Functional sensitivity analysis. Agreement between density functionals for reorganization energy calculations.}
\label{tab:functional_sensitivity}
\begin{tabular}{llcccc}
\hline
Functional 1 & Functional 2 & n & MAE (eV) & Kendall $\tau$ & p-value \\
\hline
b3lyp & camb3lyp & 6 & 0.229 & 1.000 & 0.003 \\
b3lyp & wb97x-d3 & 6 & 0.309 & 1.000 & 0.003 \\
camb3lyp & wb97x-d3 & 6 & 0.080 & 1.000 & 0.003 \\
\hline
\end{tabular}
\end{table}


==> Tables/table_orbital_composition.tex <==
% AUTO-GENERATED: Orbital composition table (n=17) - 2026-01-29
\begin{table}[h]
\centering
\caption{Nitrogen atomic contributions to frontier molecular orbitals for expanded sample. Values represent percentage contribution of all N atoms to HOMO and LUMO (n=17, GFN2-xTB + Multiwfn).}
\label{tab:orbital_composition}
\scriptsize
\begin{tabular}{lcc}
\hline
Molecule & N in HOMO (\%) & N in LUMO (\%) \\
\hline
20778 & 98.5 & 0.0 \\
24255 & 90.2 & 55.9 \\
17851 & 84.1 & 95.0 \\
12635 & 81.5 & 45.0 \\
18985 & 66.2 & 25.2 \\
14380 & 57.1 & 1.0 \\
4550 & 33.0 & 14.3 \\
20722 & 10.8 & 22.6 \\
977 & 1.5 & 2.8 \\
8521 & 1.4 & 6.7 \\
6775 & 0.8 & 10.8 \\
19531 & 0.0 & 0.0 \\
10132 & 0.0 & 0.0 \\
24524 & 0.0 & 0.0 \\
6678 & 0.0 & 0.0 \\
6966 & 0.0 & 0.0 \\
8371 & 0.0 & 0.0 \\
\hline
\multicolumn{3}{l}{\textbf{Mean $\pm$ SD (n=17):} HOMO = 30.8 $\pm$ 38.9\%, LUMO = 16.3 $\pm$ 26.4\%} \\
\multicolumn{3}{l}{\textbf{N-rich molecules (>50\% in HOMO):} 6/17 (35\%)} \\
\hline
\end{tabular}
\end{table}


==> Tables/table_orbital_composition_old_n4.tex <==
\begin{table}[h]
\centering
\caption{Nitrogen atomic contributions to frontier molecular orbitals. Values represent percentage contribution of all N atoms to HOMO and LUMO.}
\label{tab:orbital_composition}
\begin{tabular}{lcc}
\hline
Molecule & N in HOMO (\%) & N in LUMO (\%) \\
\hline
14380 & 41.6 & 0.3 \\
17851 & 76.9 & 84.7 \\
18985 & 40.5 & 18.4 \\
20778 & 79.9 & 91.4 \\
\hline
\end{tabular}
\end{table}


==> Tables/table_reorganization.tex <==
% AUTO-GENERATED: Reorganization energies table (n=13) - 2026-01-29
\begin{table}[h]
\centering
\caption{Hole reorganization energies ($\lambda_\text{hole}$) for expanded candidate set calculated using GFN2-xTB semi-empirical method. All values in eV (n=13).}
\label{tab:reorganization_energies}
\begin{tabular}{lc}
\hline
Molecule & $\lambda_\text{hole}$ (eV) \\
\hline
12635 & 0.035 \\
6775 & 0.079 \\
6966 & 0.091 \\
24255 & 0.105 \\
8371 & 0.116 \\
8521 & 0.200 \\
24524 & 0.252 \\
6678 & 0.253 \\
20778 & 0.359 \\
17851 & 0.508 \\
20722 & 0.588 \\
4550 & 0.842 \\
10132 & 1.092 \\
\hline
\multicolumn{2}{l}{\textbf{Mean $\pm$ SD (n=13):} 0.348 $\pm$ 0.325 eV} \\
\multicolumn{2}{l}{\textbf{Excellent transport ($\lambda < 0.5$ eV):} 9/13 (69\%)} \\
\hline
\end{tabular}
\end{table}


==> Tables/table_reorganization_old_n5.tex <==
\begin{table}[h]
\centering
\caption{Hole reorganization energies ($\lambda_\text{hole}$) for top candidate molecules calculated with three density functionals. All values in eV. Molecule 19531 excluded due to structural instability.}
\label{tab:reorganization_energies}
\begin{tabular}{lcccc}
\hline
Molecule & B3LYP & CAM-B3LYP & $\omega$B97X-D3 & Mean $\pm$ SD \\
\hline
20778 & -0.51 & -0.81 & -0.90 & -0.74 $\pm$ 0.21 \\
17851 & -0.25 & -0.47 & -0.53 & -0.42 $\pm$ 0.15 \\
18985 & 0.41 & 0.27 & 0.24 & 0.31 $\pm$ 0.09 \\
977 & 0.55 & 0.56 & 0.56 & 0.56 $\pm$ 0.01 \\
14380 & 0.95 & 0.82 & 0.72 & 0.83 $\pm$ 0.12 \\
\hline
\multicolumn{5}{l}{\textbf{Overall Mean (n=5):} $-0.35 \pm 0.60$ eV} \\
\hline
\end{tabular}
\end{table}


==> Tables/table_solid_state.tex <==
\begin{table}[h]
\centering
\caption{Solid-state interaction energies calculated with GFN2-xTB. Stacking energies at optimal distance and parallel-displaced dimerization energies.}
\label{tab:solid_state}
\begin{tabular}{lccc}
\hline
Molecule & Optimal Distance (\AA) & Stacking (kcal/mol) & Parallel Dimer (kcal/mol) \\
\hline
17851 & 3.2 & 5728.81 & -0.23 \\
20778 & 3.6 & 0.36 & -0.22 \\
18985 & 3.2 & -0.17 & -0.07 \\
14380 & 3.4 & -2.17 & -2.88 \\
\hline
\end{tabular}
\end{table}

